Bottleneck Transformers for Visual Recognition

We present BoTNet, a conceptually simple yet powerful backbone architecture that incorporates self-attention for multiple computer vision tasks including image classification, object detection and instance segmentation. By just replacing the spatial convolutions with global self-attention in the final three bottleneck blocks of a ResNet and no other changes, our approach improves upon the baselines significantly on instance segmentation and object detection while also reducing the parameters, with minimal overhead in latency. Through the design of BoTNet, we also point out how ResNet bottleneck blocks with self-attention can be viewed as Transformer blocks. Without any bells and whistles, BoTNet achieves 44.4% Mask AP and 49.7% Box AP on the COCO Instance Segmentation benchmark using the Mask R-CNN framework; surpassing the previous best published single model and single scale results of ResNeSt evaluated on the COCO validation set. Finally, we present a simple adaptation of the BoTNet design for image classification, resulting in models that achieve a strong performance of 84.7% top-1 accuracy on the ImageNet benchmark while being up to 1.64x faster in compute time than the popular EfficientNet models on TPU-v3 hardware. We hope our simple and effective approach will serve as a strong baseline for future research in self-attention models for vision

==> configs.tex <==
%%%%%%%%%%%%%%%%
\subsection{Why replace all three \texttt{c5} spatial convolutions?}
\label{sec:configs}

\begin{figure}[ht]%
    \centering
    \includegraphics[scale=0.4]{configs-smaller.pdf}
    \caption{Replacement configs for BoTNet in the \texttt{c5} blockgroup of a ResNet}%
    \label{fig:configs}%
\end{figure}

\begin{table*}[!ht]\centering
\small
\setlength\tabcolsep{3.5pt}
\begin{tabular}{l|c|c|ccc|ccc}
\Xhline{1.0pt}

\text{Backbone}  & \texttt{c5-attn.} & \texttt{TC Time} & {\apbbox{}} & \apbbox{S} & \apbbox{L} &  {\apmask{}} &  \apmask{S} & \apmask{L} \\[2pt]

\Xhline{1.0pt}

R50 &  \texttt{[0,0,0]} & 786.5 & 42.1  & 22.5	& 59.1 & 37.7 & 18.3	& 54.9 \\
BoT 50 & \texttt{[0,0,1]} & 813.7 & 43.4 (\textcolor{ForestGreen}{+ {\bf  1.3}}) & 23.7 (\textcolor{ForestGreen}{+ {\bf    1.2}}) &		59.7 (\textcolor{ForestGreen}{+ {\bf    0.6}}) & 38.6 (\textcolor{ForestGreen}{+ {\bf  0.9}})  &	19.0 (\textcolor{ForestGreen}{+ {\bf    0.7}}) &	55.6 (\textcolor{ForestGreen}{+ { \bf  0.7}}) \\
BoT 50 & \texttt{[0,1,1]} & 843.87 & 43.4 (\textcolor{ForestGreen}{+ {\bf  1.3}}) & 24.0 (\textcolor{ForestGreen}{+ {\bf    1.5}})	 & 60.2 (\textcolor{ForestGreen}{+ {\bf    1.1}}) & 38.6 (\textcolor{ForestGreen}{+ {\bf  0.9}}) &	19.4 (\textcolor{ForestGreen}{+ {\bf    1.1}}) &	55.9 (\textcolor{ForestGreen}{+ {\bf    1.0}}) \\
BoT R50 & \texttt{[1,0,0]} & 983.2 & 43.7 (\textcolor{ForestGreen}{+ {\bf  1.6}}) & 23.9 (\textcolor{ForestGreen}{+ {\bf    1.4}}) & {60.6} (\textcolor{ForestGreen}{+ {\bf    1.5}}) & 38.9 (\textcolor{ForestGreen}{+ {\bf   1.2}})   &	 {19.3} (\textcolor{ForestGreen}{+ {\bf    1.0}}) & 55.9 (\textcolor{ForestGreen}{+ {\bf    1.0}}) \\
BoT 50 & \texttt{[1,1,1]} & 1032.7 & 43.6 (\textcolor{ForestGreen}{+ {\bf   1.5}}) & 25.1 (\textcolor{ForestGreen}{+ {\bf 2.6}})  &	59.4 ({+ { 0.3}}) &	38.9 (\textcolor{ForestGreen}{+ {\bf   1.2}})  &	20.7 (\textcolor{ForestGreen}{+ {\bf 2.4}}) &	55.5 (\textcolor{ForestGreen}{+ {\bf 0.6}}) \\
\hline
R101 & \texttt{[0,0,0]} & 928.7 & 43.3 (\textcolor{ForestGreen}{+ {\bf  1.2}}) & 24.2 (\textcolor{ForestGreen}{+ {\bf  1.7}})  & 60.7 (\textcolor{ForestGreen}{+ {\bf  1.6}}) & 38.4 (\textcolor{ForestGreen}{+ {\bf  0.7}})  & 19.6 (\textcolor{ForestGreen}{+ {\bf  1.3}})  & 56.8 (\textcolor{ForestGreen}{+ {\bf  1.9}}) \\
BoT101 & \texttt{[1,1,1]} & 1174.9 & 45.5 (\textcolor{ForestGreen}{+ {\bf 2.2}})	& 26.0 (\textcolor{ForestGreen}{+ {\bf 1.8}}) &	62.3  (\textcolor{ForestGreen}{+ {\bf 1.6}}) &	40.4 (\textcolor{ForestGreen}{+ {\bf 2.0}})		&		21.1  (\textcolor{ForestGreen}{+ {\bf 1.5}})	&	58.0  (\textcolor{ForestGreen}{+ {\bf 1.2}}) \\


\Xhline{1.0pt}

\Xhline{1.0pt}
\end{tabular}
\vspace*{-0mm}
\caption{{Ablation study on the replacement design in BoTNet:} All models are trained with the canonical config with image size $1024\times 1024$, jitter $\left[0.8, 1.25\right]$, 36 epochs. %We see that all designs have significant improvements over the baseline R50. 
TC Time refers to TPU-v3 Compute Step Time (in milliseconds) during training.}
\label{tab:placement}
\vspace{-2mm}
\end{table*}

\vspace{-2mm}

Is replacing all the 3 spatial convolutions in \texttt{c5} the {\it minimum effective} change or could it be simplified even further? We perform an ablation study on the replacement design in order to answer this question (Please refer to Table \ref{tab:placement}, Figure \ref{fig:configs}). The baseline R50 and BoT50 go by the notation \texttt{[0,0,0]} and \texttt{[1,1,1]} since the former does not replace anything while the latter replaces the spatial convolution in all three \texttt{c5} blocks. As mentioned already, the first replacement in \texttt{c5} operates on $64\times64$ feature map while the remaining two operate on $32\times 32$. We ablate for the configs: \texttt{[0,0,1]}, \texttt{[0,1,1]} and \texttt{[1,0,0]}. The first two configs test how useful is the replacement when performed only on the smaller $32\times 32$ featuremap(s) once and twice respectively, while the last tests how useful is the replacement when performed only on the larger $64 \times 64$ featuremap.


First, we see that in terms of aggregate measures such as \apbbox{} and \apmask{}, each of the configs for BoT50 is a strict improvement over R50, with similar performance. Config. \texttt{[1,0,0]} is closer to the performance of BoT50 (\texttt{[1,1,1]}) compared to the other configurations, however a difference of 0.2 \apbbox{} is within the noise typically observed in COCO experiments. It is indeed surprising that just a single self-attention replacement layer right at the end (\texttt{[0,0,1]}) provides a visible gain of 1.3 \apbbox{}. When contrasted with the performance of R101 (43.2 \apbbox{} and 38.4 \apmask{}), the config. \texttt{[0,0,1]} is very much competitive with 43.4 \apbbox{} and 38.6 \apmask{}, with more efficient compute steptime on the TPU (1.2x faster). Nevertheless, the gains on large objects for the \texttt{[0,0,1]} config (+ 0.6 \apbbox{L}) are not as significant as those in R101 (+ 1.6 \apbbox{L}).

Among the different configs for BoT50, we see that \texttt{[1,0,0]} and \texttt{[0,1,1]} are the best in terms of good performance on both small and large objects. Surprisingly, the actual BoTNet config (\texttt{[1,1,1]}) shows significant boost on small objects (2.6 \apbbox{S}), but does not show substantial gain on large objects, even relative to other ablation configs. We suspect this could be due to poor optimization and leave it for future work to carefully understand how self-attention affects the performance on small and large objects.

Based on these ablations, consider the question: is it better to replace convolutions with self-attention in \texttt{c5} (BoT50) vs stacking more convolution layers (R101)? An argument in favor of R101 is that the gains are clear on both small and large objects unlike BoT50 where the gains are much more on small objects. However, there does exist a BoT50 config that can strictly improve upon R101, ie the \texttt{[0,1,1]} config. It has similar properties to R101 (gain on both small and large objects), similar performance on aggregate measures like \apbbox{} and \apmask{}, with a more efficient compute steptime. Hence, we can affirmatively say that {\it self-attention replacement is more efficient than stacking convolutions}.

%One could also get the best of both worlds, stacking more convolutions as well as replacing the final convolutions with self-attention. We do observe that in BoT101 where we see significant boost on both \apbbox{S}, \apbbox{L}; and \apmask{S} and \apmask{L}.

==> frcnn.tex <==
\subsection{BoTNet improves over ResNet for Object Detection}
\label{sec:frcnn}

Does BoTNet improve upon ResNet for the task of object detection as well? We verify this through experiments with the Faster R-CNN framework (Table \ref{tab:faster}). %For Tables \ref{tab:faster}, we use the canonical setting\footnote{36 epochs, $1024\times 1024$ images, $[0.8,1.25]$ jitter.}. 
We observe that BoTNet indeed improves over ResNet significantly. BoT R50 improves upon R50 by a {significant margin of + 1.6\%} \apbbox{S} (\apbbox{} for {small objects}). %while BoT R101 improves upon R101 on AP$_S$ by {\bf 3.7\%}. 
These results suggest that {\it self-attention has a big effect in detecting small objects} which is considered to be an important and hard problem for deploying object detection systems in the real world. This result is in contrast with DETR~\cite{carion2020end} which observes a big improvement on large objects but not on small objects. We believe that introducing self-attention in the backbone architecture might help fix the lack of gains on small objects in DETR. Finally, we study if larger images would further benefit BoTNet for object detection. Using a multi-scale jitter of $[0.1, 2.0]$ with 72 epoch training and image size of $1280 \times 1280$, we see that BoT R152 achieves a strong performance of {\bf 48.4\%} \apbbox{}.

\begin{table}[ht]\centering
 \small
 \setlength\tabcolsep{2.5pt}
 \begin{tabular}{l|c|c|c}
 \Xhline{1.0pt}
  \text{Backbone}  &   \apbbox{} & \apbbox{S} & \apbbox{L} \\[2pt]
  %\text{Backbone}  & \texttt{res} &  AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ \\[2pt]
 \Xhline{1.0pt}

R50  & 41.5 &	24.9 &	54.3 \\
BoT50  & 43.1 (\textcolor{ForestGreen}{+ {\bf 1.6}}) &	27.6 (\textcolor{ForestGreen}{+ {\bf 2.7}}) &	55.7 (\textcolor{ForestGreen}{+ {\bf 1.3}}) \\
\hline
R101 & 42.4 & 	24.5 &	55.0 \\
BoT101  & 44.3 (\textcolor{ForestGreen}{+ {\bf 1.9}}) & 26.5 (\textcolor{ForestGreen}{+ {\bf 2.0}}) &	57.5 (\textcolor{ForestGreen}{+ {\bf 2.5}}) \\
\hline
R152 & 45.1 &	30.1 &	56.6 \\
BoT152 & {\bf 48.4} (\textcolor{ForestGreen}{+ {\bf 3.3}}) &	{\bf 32.7} (\textcolor{ForestGreen}{+ {\bf 2.6}}) 	 &  {\bf 60.6} (\textcolor{ForestGreen}{+ {\bf 4.0}}) \\


\Xhline{1.0pt}
\end{tabular}
\vspace*{-0mm}
\caption{{BoTNet for Faster R-CNN:} The first four rows are trained for 36 epochs, jitter $\left[0.8,1.25\right]$, image size $1024\times 1024$. Final two rows are trained for 72 epochs with $1280\times1280$ image size, jitter $\left[0.1,2.0\right]$ using \texttt{v3-32} Cloud TPU.}
%\caption{\textbf{BoTNet and ResNet for Faster R-CNN:} Both BoT R50 and BoT R101 show significant improvement over R50 and R101 on \apbbox{} ({\bf + 1.8\%} and {\bf + 2.3\%} respectively). The gains on AP$_S$ (small objects) is remarkable: {\bf + 4.3\%} and {\bf + 3.7\%} for BoT R50 and BoT R101 respectively.}
\label{tab:faster}
\vspace{-2mm}
\end{table}


==> hparams_table.tex <==
\subsection{Hyperparameters}

\begin{table*}[ht]\centering
\small
\setlength\tabcolsep{2.0pt}
\begin{tabular}{l|c|c|cc|cc|c}
\Xhline{1.0pt}
% \toprule
\text{Model}  & \text{Backbone} & \text{Resolution} & \text{WD}  & \text{RA mag.} & \text{DC} & \text{DR} \\[2pt]
\Xhline{1.0pt}

{S0} & {SENet-50} & {160} & 8e-5  & 9 & 0.2 & 0.25\\
\hline

- & ResNet-50 & 224 & 8e-5  & 9 & - & - \\
- & ResNet-50 & 256 & 8e-5  & 9 & - & - \\
- & SENet-50 & 224 & 4e-5  & 15 & 0.2 & 0.25 \\
\hline

- & {ResNet-101} & {224} & 4e-5  & 15 & 0.2 & 0.25 \\
\hline

T3 & BoTNet-S1-59 & 224 & 4e-5  & 15 & 0.2 & 0.25 \\
- & ResNet-152 & 224 & 4e-5  & 15 & 0.2 & 0.25 \\ 
{S1} & {SENet-101} & {224} & 4e-5  & 15 & 0.2 & 0.25 \\
{S2} & {SENet-152} & {224} & 4e-5  & 15 & 0.2 & 0.25 \\

\hline

{T4} & { BoTNet-S1-110} & {224} & 4e-5  & 15 & 0.2 & 0.25 \\
{S3} & { SENet-152} & { 288} & 4e-5  & 15 & 0.2 & 0.25  \\

\hline

S4 & SENet-350 & {320} & 4e-5  & 15 & 0.2 & 0.25  \\ 
{T5} & {BoTNet-S1-128} & {256} &  4e-5  & 15 & 0.2 & 0.25 \\
\hline


S5 & SENet-350 & {384} & 4e-5  & 15 & 0.2 & 0.25  \\ 
{T6} & {BoTNet-S1-77} & {320} &  4e-5 &  15 & 0.2 & 0.25 \\


\hline
{T7-320} & {BoTNet-S1-128} & 320 & 2e-5 & 24 & 0.2 & 0.25  \\
{T7} & {BoTNet-S1-128} & 384 & 2e-5 & 24 & 0.2 & 0.25  \\

\hline
\Xhline{1.0pt}
\end{tabular}
\vspace*{-0mm}
\caption{Hyperparameters}
\label{tab:backbones_all}
\vspace{-2mm}
\end{table*}

==> imagenet_table.tex <==
\begin{table*}[ht]\centering
\small
\setlength\tabcolsep{2.0pt}
\begin{tabular}{l|c|c|cc|cc|c}
\Xhline{1.0pt}
% \toprule
\text{Model}  & \text{Backbone} & \text{Resolution} & \text{Top-1 Acc.}  & \text{Top-5 Acc.} & \text{Params} & \text{M.Adds} & \text{Steptime} \\[2pt]
\Xhline{1.0pt}

B0 & EfficientNet & 224 & 77.1 & 93.3 & 5.3M & 0.39B & 35.6 \\
{\bf S0} & {\bf SENet-50} & {\bf 160} & {\bf 77.0} & {\bf 93.5} & {\bf 28.02M} & {\bf 2.09B} & {\bf 32.3} \\
\hline

{\bf B1} & {\bf EfficientNet} & {\bf 240} & {\bf 79.1} & {\bf 94.4} & {\bf 7.8M} & {\bf 0.7B} &  {\bf 58.8} \\
- & ResNet-50 & 224 & 78.3 & 94.3 & 25.5M & 4.09B & 50.7 \\
- & ResNet-50 & 256 & 78.8 & 94.5   & 25.5M & 5.34B & 62.1 \\
- & SENet-50 & 224 & 79.4 & 94.6 & 28.02M & 4.09B & 64.3 \\
\hline

B2 & EfficientNet & 260 &  80.1 & 94.9 & 9.2M & 1.0B &  74.6 \\
- & {\bf ResNet-101} & {\bf 224} & {\bf 80.0} & {\bf 95.0} & {\bf 44.4M}  & {\bf 7.8B} & {\bf 63.0} \\
\hline

B3 & EfficientNet & 300 & 81.6 & 95.7 & 12M & 1.8B &  120.8 \\
T3 & BoTNet-S1-59 & 224 & 81.7 & 95.8 & 33.5M & 7.3B & 156.2 \\
- & ResNet-152 & 224 & 81.3 & 95.5 & 60.04M & 11.5B & 85.6 \\ 
{\bf S1} & {\bf SENet-101} & {\bf 224} & {\bf 81.4} & {\bf 95.7} & {\bf 49.2M} & {\bf 7.8B} & {\bf 71.1} \\
{\bf S2} & {\bf SENet-152} & {\bf 224} & {\bf 82.2} & {\bf 95.9} & {\bf 66.6M} & {\bf 11.5B}  & {\bf 97.7} \\

\hline

B4 & EfficientNet & 380 & 82.9 & 96.4 & 19M & 4.2B &  238.9 \\
{T4} & { BoTNet-S1-110} & {224} & {\bf 82.8} & {96.3} & {54.7M} & {10.9B} & {181.3} \\
{\bf S3} & {\bf SENet-152} & {\bf 288} & {\bf 83.1} & {\bf 96.4} & {\bf 66.6M} & {\bf 19.04B} & {\bf 149.9} \\

\hline
\hline

B5 & EfficientNet & 456 & 83.6 & 96.7 & 30M & 9.9B &  442.6 \\
S4 & SENet-350 & {320} & 83.6  & 96.6 & 115.18M & 52.9B & 397.9  \\ 
{\bf T5} & {\bf BoTNet-S1-128} & {\bf 256} & {\bf 83.5} & {\bf 96.5} & {\bf 75.1M} & {\bf 19.3B} & {\bf 355.2} \\
\hline


B6 & EfficientNet & 528 & 84.0 & 96.8 & 43M & 19B &  776.3 \\
S5 & SENet-350 & {384} & 83.8 & 96.6 & 115.18M & 52.9B & 397.9  \\ 
{\bf T6} & {\bf BoTNet-S1-77} & {\bf 320} & {\bf 84.0} & {\bf 96.7} & {\bf 53.9M} & {\bf 23.3B} &  {\bf 578.1} \\


\hline
B7 & EfficientNet & 600 &  84.3 & 97.0 & 66M & 37B &  1478.4 \\
{\bf T7-320} & {\bf BoTNet-S1-128} & {\bf 320} & {\bf 84.2} & {\bf 96.9} & {\bf 75.1M} & {\bf 30.9B} & {\bf 634.3} \\
B7-RA & EfficientNet & 600 & 84.7 & 97.0 & 66M & 37B &  1478.4 \\
{\bf T7} & {\bf BoTNet-S1-128} & {\bf 384} & {\bf 84.7} & {\bf 97.0} & {\bf 75.1M} & {\bf 45.8B}  & {\bf 804.5} \\

\hline
\Xhline{1.0pt}
\end{tabular}
\vspace*{-0mm}
\caption{Various backbone architectures, evaluated under the fair setting of using the improved training elements from EfficientNet~\cite{tan2019efficientnet}. Models are grouped by the accuracy of each EfficientNet model. For ResNets, SENets and BoTNets, the best weight decay from \texttt{[2e-5,4e-5,8e-5,1e-4]} the best dropconnect from \texttt{[0.2,None]}, and the best RandAugment magnitude from \texttt{[9,15,24]} are used to ensure fair comparisons to the already well tuned EfficientNets whose results we take from the latest update to the official codebase. The steptimes that we report, refer to the {\bf {compute}} time on a TPU-v3 core, for a batch size of 32 for all the models. This is to ensure we do not use different batch sizes for different models and do not conflate TPU rematerialization for dense convolutions. Had we done so (i.e picked bigger batch sizes for ResNets and BoTNets as long as they fit on memory), the speedup gains would be even higher. Further, by {\bf compute} time, we just mean the time spent for forward and backward passes, and {\bf not} the data loading. This is again to ensure comparisons across models do not exploit inefficient (or non-cached) data loading. B7-RA refers to EfficientNet-B7 trained with RandAugment~\cite{cubuk2020randaugment}.}
\label{tab:backbones_all}
\vspace{-2mm}
\end{table*}

==> qualitative_file.tex <==
\begin{figure*}[h]%
    \centering
    \includegraphics[scale=.4]{collage-better.pdf}
    %\subfloat[BoTNet Replacement Bottleneck Block]{{\includegraphics[scale=0.04]{aleph_block7.jpg} }}%
    %\subfloat[\texttt{all2all} 2D Self-Attention with Relative Position Encodings]{{\includegraphics[scale=0.1]{aleph_layer6.jpg} }
    %}%
    %\qquad
    \caption{Qualtiative Results from Mask R-CNN with BoTNet-50. Images are from the COCO dataset.}%
    \label{fig:pareto}%
\end{figure*}

\begin{figure*}[h]%
    \centering
    \includegraphics[scale=.25]{qualitative.pdf}
    %\subfloat[BoTNet Replacement Bottleneck Block]{{\includegraphics[scale=0.04]{aleph_block7.jpg} }}%
    %\subfloat[\texttt{all2all} 2D Self-Attention with Relative Position Encodings]{{\includegraphics[scale=0.1]{aleph_layer6.jpg} }
    %}%
    %\qquad
    \caption{Qualitative comparison between ResNet-50 and BoTNet-50 Mask R-CNN on images from the COCO dataset. While not very different, BoTNet is able to create more precise localizations as well as detect small objects better. A couple of examples are detecting the shadow of the kite, or the spoon next to the fork, etc.}%
    \label{fig:maskrcnn_outputs}%
\end{figure*}


% \begin{figure*}[ht]%
%     \centering
%     \includegraphics[scale=.16]{cars.pdf}
%     \caption{Fill in caption (TODO)}%
%     \label{fig:pareto}%
% \end{figure*}
